TuneComp: Joint Fine-tuning and Compression for Large Foundation Models

To reduce model size during post-training, compression methods, including knowledge distillation, low-rank approximation, and pruning, are often applied after fine-tuning the model. However, sequential fine-tuning and compression sacrifices performance, while creating a larger than necessary model as an intermediate step. In this work, we aim to reduce this gap, by directly constructing a smaller model while guided by the downstream task. We propose to jointly fine-tune and compress the model by gradually distilling it to a pruned low-rank structure. Experiments demonstrate that joint fine-tuning and compression significantly outperforms other sequential compression methods.

==> figures/table.tex <==
\begin{table*}[b]
\caption{The relationship between learning rate and ranks for LoRA based fine-tuning and PC-LoRA (joint fine-tuning and compression.)}
\label{tb_lr}
\vskip 0.15in
\begin{center}
\begin{tiny}
\begin{sc}
\begin{tabular}{lllllllllllllllll}
\toprule
\multicolumn{1}{c}{{ method}}   & \multicolumn{1}{c}{{ LR}} & {$9e^{-5}$}        & {$10^{-4}$}         & {$2e^{-4}$}         & {$3e^{-4}$}                                 & {$4e^{-4}$}         & {$5e^{-4}$}         & {$6e^{-4}$}                                 & {$7e^{-4}$}       & {$8e^{-4}$}         & {$9e^{-4}$}         & { 0.001}          & { 0.002}          & { 0.003}          & { 0.004}          & { 0.005}          \\
 \midrule
{ }                             & { 32}       & { 90.04}          & { 90.19}          & { 91.59}          & { 92.30}                                  & { 92.09}          & { \textit{92.49}} & { 92.37}                                  & { 92.41}          & { \textbf{92.54}} & { 92.39}          & { \textbf{92.61}} & { 91.98}          & { 90.27}          & { -}              & { -}              \\
 
{ }                             & { 64}       & { 90.72}          & { 90.89}          & { 92.11}          & { 92.35}                                  & { 92.38}          & { \textit{92.61}} & { \textbf{92.64}}                         & { 92.31}          & { 92.42}          & { \textbf{92.52}} & { 92.20}          & { 91.30}          & { 88.21}          & { -}              & { -}              \\
 
{ }                             & { 128}        & { 91.53}          & { 91.68}          & { 92.24}          & { \textbf{92.49}}                         & { \textit{92.46}} & { \textbf{92.49}} & { \textbf{92.59}}                         & { 92.14}          & { 92.25}          & { 92.25}          & { 91.95}          & { 87.98}          & { 88.37}          & { -}              & { -}              \\
 
\multirow{-4}{*}{{ FT}}    & { 256}       & { 92.18}          & { 92.14}          & { \textbf{92.74}} & { \textit{92.50}}                         & { \textbf{92.70}} & { 92.29}          & { 92.37}                                  & { 92.04}          & { 91.56}          & { 91.23}          & { 87.69}          & { 88.59}          & { 86.42}          & { -}              & { -}              \\ \hline
 
{ }                             & { 32} & { -}              & { 87.45}          & { 89.40}          & { 90.26}                                  & { 91.12}          & { 91.64}          & { 91.67}                                  & { 91.99}          & { 91.94}          & { \textbf{92.22}} & { 91.97}          & { \textbf{92.52}} & { \textit{92.17}} & { 92.01}          & { -}              \\
 
{ }                             & { 64}  & { -}              & { 88.16}          & { 89.95}          & { 90.78}                                  & { 91.48}          & { 91.49}          & { 91.99}                                  & { 91.80}          & { 92.11}          & { \textit{92.21}} & { 92.19}          & { \textbf{92.37}} & { \textbf{92.43}} & { 91.43}          & { -}              \\
 
{ }                             & { 128}  & { -}              & { 88.58}          & { 90.19}          & { 91.09}                                  & { 91.28}          & { 91.71}          & { 92.05}                                  & { 92.24}          & { \textbf{92.32}} & { \textbf{92.45}} & { 92.19}          & { \textit{92.29}} & { 92.17}          & { 91.55}          & { -}              \\
\multirow{-4}{*}{{ rs FT}} & { 256}& { -}              & { 89.01}          & { 90.55}          & { 91.24}                                  & { 91.53}          & { 91.85}          & { 92.14}                                  & { 92.21}          & { \textit{92.30}} & { 92.30}          & { \textbf{92.35}} & { \textbf{92.32}} & { 91.72}          & { 91.23}          & { -}              \\
\toprule
Method & LR & {$7e^{-5}$}& {$8e^{-5}$}& {$9e^{-5}$}        & {$10^{-4}$}         & {$2e^{-4}$}         & {$3e^{-4}$}                                 & {$4e^{-4}$}         & {$5e^{-4}$}         & {$6e^{-4}$}                                 & {$7e^{-4}$}       & {$8e^{-4}$}         & {$9e^{-4}$}      & { 0.001}          & { 0.002}          & { 0.003}         \\
\midrule
{ }                             & { 32}                                                        & { 57.64}          & { 59.52}     & { 60.84}          & { 61.26}          & { 69.79}          & { 73.90}                                  & { 75.32}          & { 76.55}          & { 76.88}                                  & { \textbf{78.21}} & { \textit{78.09}} & { 77.96}          & { \textbf{78.39}} & { 77.83}          & { 75.54}   \\
{ }                             & { 64}                                                        & { 76.86}          & { 77.43}     & { 78.47}          & { 79.24}          & { 82.32}          & { 83.11}                                  & { 83.69}          & { 83.93}          & { \textbf{84.27}} & { \textbf{84.07}} & { 83.73}          & { \textbf{84.07}} & { 83.89}          & { 81.47}          & { 79.43}  \\
{ }                             & { 128}                                                       & { 86.66}          & { 86.79}     & { 86.82}          & { 87.08}          & { \textbf{87.79}} & { \textbf{88.12}} & { \textit{87.44}} & { 87.30}          & { 87.17}                                  & { 87.05}          & { 86.38}          & { 86.71}          & { 86.02}          & { 82.80}          & { 81.29} \\
\multirow{-4}{*}{{ PC-LoRA}}    & { 256}                                                       & { \textit{90.54}} & { 90.34}     & { \textbf{90.80}} & { \textbf{90.75}} & { 90.16}          & { 89.54}                                  & { 89.58}          & { 88.43}          & { 87.93}                                  & { 87.44}          & { 87.28}          & { 86.72}          & { 86.17}          & { 83.02}          & { -}  \\
\toprule
Method & LR & {$9e^{-5}$}        & {$10^{-4}$}         & {$2e^{-4}$}         & {$3e^{-4}$}                                 & {$4e^{-4}$}         & {$5e^{-4}$}         & {$6e^{-4}$}                                 & {$7e^{-4}$}       & {$8e^{-4}$}         & {$9e^{-4}$}     & { 0.001}          & { 0.002}          & { 0.003}   & { 0.004} & { 0.005}       \\
\midrule
{ }                             & { 32}   & { -}              & { 26.85}          & { 38.27}          & { 47.61}                                  & { 52.41}          & { 58.68}          & { 57.52}                                  & { 61.77}          & { 66.44}          & { 66.05}          & { 65.90}          & { \textit{70.74}} & { 70.35}          & { \textbf{71.62}} & { \textbf{74.96}} \\
{ }                             & { 64}    & { -}              & { 29.63}          & { 42.82}          & { 49.73}                                  & { 59.15}          & { 61.11}          & { 63.35}                                  & { 67.54}          & { 69.44}          & { 70.00}          & { 69.98}          & { \textbf{76.59}} & { \textit{76.50}} & { \textbf{77.99}} & { 73.75}          \\
{ }                             & {128}    & { -}              & { 30.28}          & { 44.40}          & { 53.17}                                  & { 58.77}          & { 63.74}          & { 69.24}                                  & { 68.62}          & { 71.82}          & { 73.09}          & { 74.86}          & { \textit{77.99}} & { 77.64}          & { \textbf{78.60}} & { \textbf{79.34}} \\
\multirow{-4}{*}{{ rs PC-LoRA}} & {256}    & { -}              & { 31.75}          & { 47.26}          & { 54.60}                                  & { 61.68}          & { 65.22}          & { 65.35}                                  & { 70.30}          & { 69.77}          & { 72.79}          & { 74.54}          & { 75.92}          & { \textbf{80.22}} & { \textbf{78.84}} & { \textit{78.71}} \\
\bottomrule
\end{tabular}
\end{sc}
\end{tiny}
\end{center}
\vskip -0.1in
\end{table*}
